3DLabelProp: Geometric-Driven Domain Generalization for LiDAR Semantic Segmentation in Autonomous Driving

Domain generalization aims to find ways for deep learning models to maintain their performance despite significant domain shifts between training and inference datasets. This is particularly important for models that need to be robust or are costly to train. LiDAR perception in autonomous driving is impacted by both of these concerns, leading to the emergence of various approaches. This work addresses the challenge by proposing a geometry-based approach, leveraging the sequential structure of LiDAR sensors, which sets it apart from the learning-based methods commonly found in the literature. The proposed method, called 3DLabelProp, is applied on the task of LiDAR Semantic Segmentation (LSS). Through extensive experimentation on seven datasets, it is demonstrated to be a state-of-the-art approach, outperforming both naive and other domain generalization methods.

==> src/8.lmos.tex <==
\section{Domain generalization in LiDAR Moving Object Segmentation (LMOS)}

\subsection{3DLabelProp for LMOS}


\begin{table*}[h]
    \centering
    \begin{tabular}{l|ccccl}
        \multicolumn{1}{c}{Name} & \# scans & \# fibers (sensor) & Use for training & Use for evaluation & \multicolumn{1}{c}{Specificities} \\\midrule\hline
        SemanticKITTI \cite{semantickitti} train & 20000& 64 & \checkmark & $\times$ & Few moving objects \\ \hline
        SemanticKITTI \cite{semantickitti} val (SK val)& 4000 & 64 & \checkmark & \checkmark & N/A\\ \hline
        SemanticKITTI \cite{semantickitti} test (SK test) & 20000 & 64 & $\times$& \checkmark & N.A \\ \hline
        SemanticKITTI-Tracking \cite{semantickitti} (SKT)& 1000& 64 & $\times$& \checkmark & Many moving objects   \\ \hline
        Apollo \cite{lu2019l3} (AP) & 6600& 64 & $\times$& \checkmark & N.A  \\ \hline
%        nuScenes \cite{nuscenes} train  & 18000 & 32 & \checkmark& $\times$ & Many moving objects \\ \hline
        nuScenes \cite{nuscenes} val (NS) & 6000 & 32 & $\times$& \checkmark & Many moving objects \\\hline\midrule
    \end{tabular}
    \caption{MOS dataset informations.}
    \label{tab:mos_data}
\end{table*}


In the Related works section we introduced what is MOS and some of the flagship methods. Contrary to semantic segmentation, due to the nature of the classes, MOS methods already leverage the sequentiality of the data. As a result, 3DLabelProp already fits in the mould of the task.

Nonetheless, it requires a few tweaks to be applied to MOS. We can distinguish two strategies: semantic MOS and binary MOS. Semantic MOS corresponds to SemanticKITTI's multi-frame benchmark and consists in performing the semantic segmentation over 25 classes, rather than 19, and in differentiating each type of movable object between static and moving. Binary MOS is the typical mos annotation which only distinguish static from moving objects.

Due to the sparse nature of the MOS annotations, it is necessary to change some geometric parameters. First the number of extracted cluster is decreased to $N_c$=5. Indeed, as propagation is performed on all static objects and that we can the possibility to know which vehicles are moving and which are not, the propagation is done on most of the points. Resulting in very few residual points. $V_c$, the size of the neighborhoods, is decreased as it consists mainly in static points which we do not need for segmentation. 

Furthermore, we introduce the use of a timestamp as an input feature which is added to the occupancy. A very simple timestamp information is added, as it is set at -1 for past frames, belonging to the reference cloud, and +1 for the current segmented frame. In \autoref{tab:timestamp}, we highlight the effectiveness of this feature for MOS generalization.

\begin{table}[h]
    \centering
    \begin{tabular}{l|cccc}
        \multicolumn{1}{c}{Model}& SK val & NS & AP & SKT \\\midrule\hline
        3DLabelProp &\textbf{79,0} & 39,3 & 72,3 & 65,8\\\hline
        3DLabelProp w/ \underline{timestamp} &78,4 &  \textbf{41,6} & \textbf{76,3} & \textbf{71,2} \\ \midrule \hline
    \end{tabular}
    \caption{Influence of the timestamp as an input feature for MOS. Results are computed on SemanticKITTI (SK), nuScenes (NS), Apollo (AP) and SemanticKITTI-Tracking (SKT).}
    \label{tab:timestamp}
\end{table}




\subsection{Datasets}

Traditionally, there are 3 datasets for LiDAR MOS: SemanticKITTI, Apollo and nuScenes. SemanticKITTI and nuScenes were already introduced for semantic segmentation. It is usually SemanticKITTI that is used for training, and other datasets for evaluation.

Apollo is a subset of a SLAM and object detection dataset that was annotated for MOS. It was acquired with the same sensor as SemanticKITTI, which results in minor \underline{sensor shift}.

To further study the reliability and generalization performances of MOS methods, \cite{mersch2023building} annotated a test sequence of SemanticKITTI for MOS. This novel dataset is called SemanticKITTI-Tracking and was selected due to the high number of dynamic objects, contraty to other SemanticKITTI sequences. It results in a high \underline{scene shift} relatively to SemanticKITTI.

All the aforementioned datasets information are summarized in \autoref{tab:mos_data}. It can be noted that nuScenes is the only dataset with a sensible sensor shift.


\subsection{Generalization results}

MOS methods already studied domain generalization performances. Especially, 4DMOS and MapMOS provided a first domain generalization benchmark, which is reported in \autoref{tab:gene}. In addition, we added 3DLabelProp results.

Methods that were designed without taking into account generalization (LMNet and MotionSeg3D) reach very poor generalization performances, even on Apollo which has almost no sensor shift compare to SemanticKITTI.

MapMOS and 4DMOS were designed to take into account domain generalization and are the main point of comparison that we have.

4DMOS reached the highest performances on nuScenes, which is the hardest generalization case for MOS due to the change in resolution and scene type. MapMOS reached the highest performances for SemanticKITTI-Tracking and Apollo. It can be considered the most promising domain generalization method. Nonetheless, we can see that both of them fall short on the source-to-source case as they reach lower performances on SemanticKITTI test than MotionSeg3D.

3DLabelProp provides on-par results with the state-of-the-art even though it was not designed for MOS. It reaches the second best performances on SemanticKITTI test, highlighting its relevance in source-to-source segmentation and on nuScenes and Apollo, highlighting its resilience to domain shifts.

While not being as convincing for MOS as it is for semantic segmentation, we can see that a pseudo-dense approach can be considered for MOS domain generalization as well. It demonstrates that meaningful time-realted information can be extracted from pseudo-dense pointclouds.
 
\begin{table}[h]
    \centering
    \begin{tabular}{l|ccccc}
        \multicolumn{1}{c}{Model}& SK val & SK test& NS & AP & SKT \\\midrule\hline
        LMNet \cite{LMNET}& 63,8 &62,5& N/A& 13,7 & 45,3\\ \hline
        MotionSeg3D \cite{sun2022efficient}&71,4&\textbf{70,2}&N/A &8,8 & 54,8\\ \hline
        4DMOS \cite{4DMOS} &77,2 & 65,2&\textbf{44,8} & 73,1& \underline{75,5} \\ \hline
        MapMOS \cite{mersch2023building}&\textbf{86,1} & 66,0&40,3 & \textbf{81,7}& \textbf{78,4}\\\hline

        %RVMOS \cite{RVMOS}& 71,2  &\textbf{74,7}& N/A & N/A & N/A \\ \hline
        \tabcell{3DLabelProp Binary} &\underline{78,4}& \underline{67,0} & \underline{41,6}& 76,3& 71,2 \\\hline
        \tabcell{3DLabelProp Semantic} &N/A*&64,0 & 35,0&\underline{79,8} &54,7\\ \hline \midrule
    \end{tabular}
    \caption{MOS domain generalization performances. All models were trained on SemanticKITTI. *3DLabelProp Semantic use the sequence 08 for training in order to be exposed to moving motorcyclists and moving bicyclists.}
    \label{tab:gene}
\end{table}


